Monte Carlo Simulation of Charge Transport in Graphene (Simulazione Monte Carlo per il trasporto di cariche nel grafene)

Simulations of charge transport in graphene are presented by implementing a recent method published on the paper: V. Romano, A. Majorana, M. Coco, "DSMC method consistent with the Pauli exclusion principle and comparison with deterministic solutions for charge transport in graphene", Journal of Computational Physics 302 (2015) 267-284. After an overview of the most important aspects of the semiclassical transport model for the dynamics of electrons in monolayer graphene, it is made a comparison in computational time between MATLAB and Fortran implementations of the algorithms. Therefore it is studied the case of graphene on substrates which it is produced original results by introducing models for the distribution of distances between graphene's atoms and impurities. Finally simulations, by choosing different kind of substrates, are done. ----- Le simulazioni per il trasporto di cariche nel grafene sono presentate implementando un recente metodo pubblicato nell'articolo: V. Romano, A. Majorana, M. Coco, "DSMC method consistent with the Pauli exclusion principle and comparison with deterministic solutions for charge transport in graphene", Journal of Computational Physics 302 (2015) 267-284. Dopo una panoramica sugli aspetti pi\`u importanti del modello di trasporto semiclassico per la dinamica degli elettroni nel grafene sospeso, \`e stato effettuato un confronto del tempo computazionale tra le implementazioni MATLAB e Fortran dell'algoritmo. Inoltre \`e stato anche studiato il caso del grafene su substrato su cui sono stati prodotti dei risultati originali considerando dei modelli per la distribuzione delle distanze tra gli atomi del grafene e le impurezze. Infine sono state effettuate delle simulazioni scegliendo substrati di diversa natura.

==> Chapters/Chapter4.tex <==
\section{La meccanica statistica}\label{PAR:CAP1:Meccanica_statistica}

%http://www.mat.unimi.it/users/carati/didattica/dispense/hamilton.pdf

Si consideri un sistema meccanico hamiltoniano definito da una varietà (ad esempio lo spazio $\mathbb{R}^{6N}$) sulla quale sia assegnata un'equazione differenziale
\begin{equation}
\dot{\mathbf{x}}=\mathbf{v}(\mathbf{x}),
\end{equation}
dove $\mathbf{x}=(\mathbf{q},\mathbf{p})$ sono le coordinate hamiltoniane e $\mathbf{v}=\mathbf{v}(\mathbf{x})$ è un campo vettoriale assegnato sulla varietà che presenta la struttura hamiltoniana
\begin{equation}
\mathbf{v} = \mathbb{E} \cdot \nabla \mathcal{H},
\end{equation}
con una fissata hamiltoniana $H$.\\
Lo stato di un sistema meccanico è definito da un punto nello spazio delle fasi. Assegnando le forze (ovvero l'hamiltoniana) e lo stato iniziale si ottiene l'evoluzione del sistema in modo deterministico. Uno stato di questa tipologia si dice \textbf{stato microscopico}. Se il sistema è costituito da un grande numero di particelle (come nel caso di un gas, in cui il numero di gradi di libertà è dell'ordine del numero di Avogadro, cioè circa $10^{23}$) risulta praticamente impossibile studiare gli stati microscopici. Si passa allora ad una descrizione termodinamica, in cui lo stato di un gas viene definito assegnando due sole variabili ovvero la temperatura e il volume in cui è racchiuso. In tal caso si parla di \textbf{stato macroscopico}.

La \textbf{meccanica statistica} nasce con lo scopo di creare una via di mezzo tra le due nozioni di stato, introducendo concetti di tipo probabilistico o statistico. La nozione più adatta a questo ruolo è quella di \textbf{stato statistico}. Si procede considerando il modello microscopico e assegnando una probabilità ai dati iniziali dello spazio delle fasi (ulteriori dettagli sulla definizione della densità saranno trattati nel Paragrafo \ref{PAR:CAP1:Teoria_Cinetica}). Si osservi che tale spazio è un insieme continuo e di conseguenza è necessario introdurre una densità di probabilità $\rho_0(\mathbf{x})$ con le proprietà
\begin{equation}
\rho_0 \geq 0, \qquad \int \! \rho_0 \,\diff V =1,
\end{equation}
dove $\diff V$ è l'elemento di volume nello spazio delle fasi definito da
\begin{equation}
\diff V = \diff q_1\cdots\diff q_n \diff p_1\cdots\diff p_n.
\end{equation}
Allora la probabilità che lo stato del sistema si trovi inizialmente in un arbitrario dominio $D_0$ dello spazio delle fasi è data da
\begin{equation}
p \left( \mathbf{x}\in D_0 \right) =\int_{D_0} \! \rho_0(\mathbf{x}) \,\diff V.
\end{equation}
Se $f=f(\mathbf{x})$ è una variabile dinamica si può definire il \textbf{valore medio} come la generalizzazione della media pesata di tutti i possibili stati microscopici iniziali, cioè
\begin{equation}
< f >_{\rho_0} = \int \! \rho_0(\mathbf{x})f(\mathbf{x}) \,\diff V.
\end{equation}
A questo punto si potrà calcolare la varianza e la distribuzione di probabilità di $f$ come usualmente accade nella teoria della probabilità.

Si supponga che il sistema sia descritto al variare del tempo $t$ da uno stato statistico, cioè da una densità di probabilità
\begin{equation}
\rho = \rho (\mathbf{x},t)
\end{equation}
e imponendo che la probabilità che il sistema si trovi al tempo $t$ nel dominio $D$ sia data da
\begin{equation}
p \left( \mathbf{x}\in D \right) =\int_{D} \! \rho(\mathbf{x},t) \,\diff V.
\end{equation}
Data la condizione di raccordo $\rho(\mathbf{x},0)=\rho_0(\mathbf{x})$ ed essendo $D(t)$ l'evoluzione al tempo $t$ del dominio $D_0$, si ha la condizione di compatibilità
\begin{equation}\label{EQ:CAP1:Cond_comp}
\int_{D(t)} \! \rho(\mathbf{x},t) \,\diff V = \int_{D_0} \! \rho_0(\mathbf{x}) \,\diff V, \qquad \forall D_0, \, \forall t.
\end{equation}
Essendo il secondo membro una costante fissati di volta in volta $D_0$ e $t$, si ha che la \eqref{EQ:CAP1:Cond_comp} è equivalente a
\begin{equation}
\frac{\diff}{\diff t} \int_{D(t)} \! \rho(\mathbf{x},t) \,\diff V = 0,
\end{equation}
cioè la densità $\rho$ è un invariante integrale. Inoltre tale condizione può essere espressa equivalentemente con una condizione di tipo differenziale. Cioè è possibile dimostrare (cfr. \citep{DISP:Carati}) che la condizione di compatibilità implica che la densità deve soddisfare la seguente equazione differenziale
\begin{equation}
\frac{\partial \rho}{\partial t} + \nabla \cdot (\rho\mathbf{v}) =0,
\end{equation}
detta \textbf{equazione di continuità}.

Inoltre dall'identità
\begin{equation}
\nabla \cdot (\rho \mathbf{v}) = \rho \nabla \cdot \mathbf{v} + \mathbf{v} \cdot \nabla \rho
\end{equation}
e dalla \eqref{EQ:CAP1:Struttura_v} per cui si ha \eqref{EQ:CAP1:Cond_solenoidale}, segue che l'equazione di continuità assume la forma
\begin{equation}\label{EQ:CAP1:Liouville_2}
\frac{\partial \rho}{\partial t} + \mathbf{v} \cdot \nabla \rho =0,
\end{equation}
o equivalentemente
\begin{equation}\label{EQ:CAP1:Liouville}
\frac{\partial \rho}{\partial t} + \left\lbrace \rho,H \right\rbrace  =0.
\end{equation}
Grazie al Teorema \ref{TEOR:CAP1:Costante_moto_ver2} ciò è equivalente al fatto che la densità sia una costante del moto. Quando quest'ultima equazione è pensata in relazione agli stati statistici anziché alle variabili dinamiche prende il nome di \textbf{equazione di Liouville}.
\begin{osservazione}
Ritornando alle coordinate hamiltoniane, ricordando la posizione $\mathbf{x}=(\mathbf{q},\mathbf{p})$, si ha che $\mathbf{v}=(\dot{\mathbf{q}},\dot{\mathbf{p}})$ e di conseguenza l'equazione \eqref{EQ:CAP1:Liouville_2} si può scrivere
\begin{equation}\label{EQ:CAP1:Liouville_3}
\frac{\partial \rho}{\partial t} + (\mathbf{q},\mathbf{p}) \cdot \nabla \rho =0.
\end{equation}
Inoltre, ponendo
\begin{equation}
\nabla_{\mathbf{q}} \: \rho =\left( \frac{\partial \rho}{\partial q_1},\ldots,\frac{\partial \rho}{\partial q_n}\right) , \quad \nabla_{\mathbf{p}} \: \rho =\left( \frac{\partial \rho}{\partial p_1},\ldots,\frac{\partial \rho}{\partial p_n}\right)
\end{equation}
la \eqref{EQ:CAP1:Liouville_3} diventa
\begin{equation}\label{EQ:CAP1:Liouville_4}
\frac{\partial \rho}{\partial t} + \mathbf{q} \cdot \nabla_{\mathbf{q}} \: \rho + \mathbf{p} \cdot \nabla_{\mathbf{p}} \: \rho =0.
\end{equation}
\end{osservazione}

%----------------------------------------------------------------------------------------

\section{La teoria cinetica dei gas}\label{PAR:CAP1:Teoria_Cinetica}

La \textbf{teoria cinetica dei gas} studia le proprietà macroscopiche di un gran numero di particelle partendo dalle loro equazioni del moto. 

Si consideri un gas costituito da $N$ molecole monoatomiche. Si assume che lo stato di una molecola è determinato completamente dalle componenti del vettore posizione e dalle componenti del vettore velocità di traslazione, si ignora cioè la possibile eccitazione dovuta ai gradi di libertà interni (rotazionale, vibrazionale ed elettronica). Si supponga che le molecole siano identiche. Se sono assegnate le posizioni e le velocità di tutte le molecole al tempo $t=0$, allora l'andamento successivo del sistema è determinato completamente da un sistema di $N$ leggi di Newton.

Nella pratica il numero di queste equazioni è enorme (in $1\,\si{\centi\metre}^3$ di gas a pressione atmosferica ci sono circa $10^{19}$ molecole). Quindi è opportuno procedere con una descrizione statistica dell'andamento del sistema.

Introducendo il formalismo hamiltoniano, ad ogni istante $t$, lo stato microscopico del sistema delle $N$ particelle è descritto specificando la posizione $\vec{q}_i(t)$ e il momento $\vec{p}_i(t)$ di ogni particella del sistema. Si ottiene in questo caso uno spazio delle fasi a $6N$ dimensioni che sarà indicato con $\Gamma$. Ad ogni istante $t$, lo stato microscopico del sistema è rappresentato da un punto di $\Gamma$. Allora l'evoluzione del sistema è governato dalle equazioni di Hamilton
\begin{equation}\label{EQ:CAP1:Sistema_Hamilton_gas}
\left\lbrace 
\begin{aligned}
\frac{\diff \vec{q}_i}{\diff t} & = \frac{\partial \mathcal{H}}{\partial \vec{p}_i} \\
\frac{\diff \vec{q}_i}{\diff t} & = -\frac{\partial \mathcal{H}}{\partial \vec{q}_i}
\end{aligned}
\right.
\end{equation}
dove l'hamiltoniana $\mathcal{H}(\mathbf{q},\mathbf{p})$ descrive l'energia totale in termini dell'insieme delle posizioni $\mathbf{q} = \left\lbrace \vec{q}_1,\ldots,\vec{q}_N \right\rbrace $ e dell'insieme dei momenti $\mathbf{p} = \left\lbrace \vec{p}_1,\ldots,\vec{p}_N \right\rbrace $.

Si osservi che uno stato macroscopico può essere rappresentato da un gran numero di stati microscopici. Questo suggerisce l'introduzione degli stati statistici. Si considerino $\mathcal{N}$ copie di un particolare stato macroscopico, ciascuna descritta da un diverso stato microscopico, ovvero da un diverso punto rappresentativo dello spazio delle fasi $\Gamma$. Sia $\diff \mathcal{N}(\mathbf{q},\mathbf{p},t)$ il numero di punti rappresentativi in un volume infinitesimo $\diff \Gamma = \prod_{i=1}^N \diff^3 \vec{q}_i \diff^3 \vec{p}_i$ costruito attorno al punto $(\mathbf{q},\mathbf{p})$. La densità dello spazio delle fasi è definita allora da
\begin{equation}
\rho (\mathbf{q},\mathbf{p},t) \diff \Gamma = \lim_{\mathcal{N}\to +\infty} \frac{\diff \mathcal{N}(\mathbf{q},\mathbf{p},t)}{\mathcal{N}}.
\end{equation}
A questo punto sono valide tutte le proprietà per la densità descritte nel Paragrafo \ref{PAR:CAP1:Meccanica_statistica}.

\section{La gerarchia BBGKY}\label{PAR:CAP1:Gerarchia_BBGKY}

In primo luogo è opportuno concentrarsi, piuttosto che sulla funzione densità a $N$ molecole, su quella a una molecola. Ad esempio, fissando la particella che occupa lo stato $(\vec{q}_1,\vec{p}_1)$ tale distribuzione si ottiene integrando su tutti i possibili valori di $\vec{q}_1$ e $\vec{p}_1$. Inoltre, assumendo che la densità sia simmetrica rispetto alle permutazioni di molecole, si ha
\begin{equation}
f_1(\vec{q},\vec{p},t) = N \int \! \rho(\vec{q}_1=\vec{q},\vec{q}_2,\ldots,\vec{q}_N,\vec{p}_1=\vec{p},\vec{p}_2,\ldots,\vec{p}_N,t) \, \prod_{i=2}^N \diff V_i ,
\end{equation}
dove $\diff V_i = \diff^3 \vec{q}_i \diff^3 \vec{p}_i$. Analogamente, la funzione densità a due molecole è data da
\begin{equation}
f_2(\vec{q}_1,\vec{q}_2,\vec{p}_1,\vec{p}_2,t) = N(N-1) \int \! \rho(\vec{q}_1,\vec{q}_2,\ldots,\vec{q}_N,\vec{p}_1,\vec{p}_2,\ldots,\vec{p}_N,t) \, \prod_{i=3}^N \diff V_i,
\end{equation}
dove la quantità $N(N-1)$ è il numero di modi in cui è possibile scegliere $2$ molecole in un insieme di $N$. Si osservi che l'integrazione al secondo membro è effettuata sulle variabili $\vec{q}_3,\ldots,\vec{q}_N,\vec{p}_3,\ldots,\vec{p}_N$. In generale, la funzione densità a $s$ molecole è data da
\begin{equation}\label{EQ:CAP1:Densita_s_particelle}
\begin{aligned}
f_s(\vec{q}_1,\ldots,\vec{q}_s,\vec{p}_1,\ldots,\vec{p}_s,t) &= \frac{N!}{(N-s)!} \int \! \rho(\mathbf{q},\mathbf{p},t) \, \prod_{i=s+1}^N \diff V_i=\\
& = \frac{N!}{(N-s)!} \rho_s(\vec{q}_1,\ldots,\vec{q}_s,\vec{p}_1,\ldots,\vec{p}_s,t),
\end{aligned}
\end{equation}
dove $\rho_s$ è la densità dello spazio delle fasi in cui sono libere le coordinate di una $s$-upla di molecole e che si ottiene integrando $\rho$ sulle coordinate delle $N-s$ molecole rimanenti. Infine si ha $\rho_N\equiv\rho$.

L'evoluzione delle $\rho_s$ è governata dalla \textbf{gerarchia di equazioni BBGKY} attribuita a Bogoliubov, Born, Green, Kirkwood, and Yvon. Nell'ambito della teoria cinetica dei gas si fa uso della seguente hamiltoniana, la quale descrive adeguatamente i gas debolmente interagenti e ha la forma
\begin{equation}
\mathcal{H}(\mathbf{q},\mathbf{p}) = \sum_{i=1}^N \left[ \frac{{\vec{p}_i}^{\; 2}}{2m} + \mathcal{U}\left( \vec{q}_i \right)  \right] + \frac{1}{2} \sum_{i,j=1}^N \mathcal{V} \left( \vec{q}_i-\vec{q}_j \right),
\end{equation}
dove $m$ è la massa di una singola particella, $\mathcal{U}$ è un potenziale esterno e $\mathcal{V}$ è un potenziale che considera le interazione tra due molecole.

Per valutare l'evoluzione nel tempo delle $f_s$ è opportuno suddividere l'hamiltoniana in
\begin{equation}
\mathcal{H}=\mathcal{H}_s+\mathcal{H}_{N-s}+\mathcal{H}',
\end{equation}
dove $\mathcal{H}_s$ e $\mathcal{H}_{N-s}$ includono le interazioni tra ogni gruppo di particelle, con
\begin{equation}
\mathcal{H}_s = \sum_{n=1}^s \left[ \frac{{\vec{p}_n}^{\; 2}}{2m} + \mathcal{U}\left( \vec{q}_n \right)  \right] + \frac{1}{2} \sum_{n,m=1}^s \mathcal{V} \left( \vec{q}_n-\vec{q}_m \right),
\end{equation}
\begin{equation}
\mathcal{H}_{N-s} = \sum_{i=s+1}^N \left[ \frac{{\vec{p}_i}^{\; 2}}{2m} + \mathcal{U}\left( \vec{q}_i \right)  \right] + \frac{1}{2} \sum_{i,j=s+1}^N \mathcal{V} \left( \vec{q}_i-\vec{q}_j \right),
\end{equation}
e le interazioni tra le molecole contenute in
\begin{equation}
\mathcal{H}'= \sum_{n=1}^s \sum_{i=s+1}^N \mathcal{V} \left( \vec{q}_n-\vec{q}_i \right).
\end{equation}
Dalla \eqref{EQ:CAP1:Densita_s_particelle} e dalla \eqref{EQ:CAP1:Liouville} si ha che l'evoluzione nel tempo delle $f_s$ può essere ottenuta calcolando
\begin{equation}\label{EQ:CAP1:Evoluzione_rho_s}
\frac{\partial \rho_s}{\partial t} = \int \! \frac{\partial \rho}{\partial t} \, \prod_{i=s+1}^N \diff V_i = - \int \! \left\lbrace \rho,\mathcal{H}_s+\mathcal{H}_{N-s}+\mathcal{H}' \right\rbrace  \, \prod_{i=s+1}^N \diff V_i,
\end{equation}
in cui le parentesi di Poisson all'ultimo membro possono essere calcolate separatamente in virtù della proprietà \ref{PTA:CAP1:Parentesi_Poisson_pta_2} della Proposizione \ref{PROP:CAP1:Parentesi_Poisson}.

Poiché l'integrazione non riguarda le prime $s$ coordinate allora è possibile scambiare il segno di integrale e le parentesi di Poisson nel primo termine che si viene a creare applicando la proprietà \ref{PTA:CAP1:Parentesi_Poisson_pta_2} della Proposizione \ref{PROP:CAP1:Parentesi_Poisson} nella \eqref{EQ:CAP1:Evoluzione_rho_s}, cioè si ha
\begin{equation}\label{EQ:CAP1:Evoluzione_H_s}
\int \! \left\lbrace \rho,\mathcal{H}_s \right\rbrace  \, \prod_{i=s+1}^N \diff V_i = \left\lbrace \left( \int \! \rho \, \prod_{i=s+1}^N \diff V_i \right),\mathcal{H}_s  \right\rbrace = \left\lbrace  \rho_s,\mathcal{H}_s\right\rbrace .
\end{equation}
Per quanto riguarda il secondo termine della \eqref{EQ:CAP1:Evoluzione_rho_s}, scrivendo esplicitamente le parentesi di Poisson e integrando successivamente per parti, si ottiene
\begin{equation}\label{EQ:CAP1:Evoluzione_H_N_s}
-\int \! \left\lbrace \rho,\mathcal{H}_{N-s} \right\rbrace  \, \prod_{i=s+1}^N \diff V_i = 0.
\end{equation}
Infine, per quanto riguarda il terzo termine della \eqref{EQ:CAP1:Evoluzione_rho_s}, scrivendo esplicitamente le parentesi di Poisson, suddividendo la sommatoria, integrando per parti e semplificando si ha
\begin{equation}\label{EQ:CAP1:Evoluzione_H_primo}
-\int \! \left\lbrace \rho,\mathcal{H}' \right\rbrace \, \prod_{i=s+1}^N \diff V_i = (N-s) \sum_{n=1}^s \int \! \diff V_{s+1} \frac{\partial \mathcal{V}(\vec{q}_n-\vec{q}_{s+1})}{\partial \vec{q}_n} \cdot \frac{\partial \rho_{s+1}}{\partial \vec{p}_n}
\end{equation}
(ulteriori dettagli su come ottenere \eqref{EQ:CAP1:Evoluzione_H_N_s} e \eqref{EQ:CAP1:Evoluzione_H_primo} sono presenti in \citep{BOOK:Kardar}).

Allora, sommando \eqref{EQ:CAP1:Evoluzione_H_s}, \eqref{EQ:CAP1:Evoluzione_H_N_s} e \eqref{EQ:CAP1:Evoluzione_H_primo} e sostituendo nella \eqref{EQ:CAP1:Evoluzione_rho_s}, si ha
\begin{equation}\label{EQ:CAP1:Gerarchia_BBGKY_rho}
\frac{\partial \rho_s}{\partial t} - \left\lbrace \mathcal{H}_s,\rho_s \right\rbrace = (N-s) \sum_{n=1}^s \int \! \diff V_{s+1} \frac{\partial \mathcal{V}(\vec{q}_n-\vec{q}_{s+1})}{\partial \vec{q}_n} \cdot \frac{\partial \rho_{s+1}}{\partial \vec{p}_n},
\end{equation}
oppure in termini delle densità $f_s$,
\begin{equation}
\frac{\partial f_s}{\partial t} - \left\lbrace \mathcal{H}_s,f_s \right\rbrace = \sum_{n=1}^s \int \! \diff V_{s+1} \frac{\partial \mathcal{V}(\vec{q}_n-\vec{q}_{s+1})}{\partial \vec{q}_n} \cdot \frac{\partial f_{s+1}}{\partial \vec{p}_n},
\end{equation}
ottenendo così la gerarchia di equazioni cercata. Infatti $\partial \rho_1 / \partial t$ dipende da $\partial \rho_2 / \partial t$, la quale dipende da $\partial \rho_3 / \partial t$ e così via.

Si può osservare che in assenza di interazioni con le altre molecole, si ha
\begin{equation}
\frac{\partial \rho_s}{\partial t} - \left\lbrace \mathcal{H}_s,\rho_s \right\rbrace = 0.
\end{equation}
Invece, se si considerano le interazioni con le rimanenti $N-s$ molecole, il termine al secondo membro della \eqref{EQ:CAP1:Gerarchia_BBGKY_rho} prende il nome di \textbf{termine collisionale} ed è costituito dai contributi forniti dal potenziale di collisione di ciascuna delle $s$ molecole del gruppo con le $N-s$ molecole restanti.

\section{L'equazione di Boltzmann}

Si vuole determinare un sistema chiuso di equazioni per la $f_1$ della gerarchia \eqref{EQ:CAP1:Gerarchia_BBGKY_rho}. Allo scopo, si considerino le prime due equazioni della gerarchia, poi si scrivano esplicitamente le parentesi di Poisson e si supponga che il potenziale $\mathcal{V}$ sia simmetrico, cioè $\mathcal{V}(\vec{q}_1 - \vec{q}_2) = \mathcal{V}(\vec{q}_2-\vec{q}_1)$, quindi si ha
\begin{equation}
\left[ \frac{\partial}{\partial t} - \frac{\partial \mathcal{U}}{\partial \vec{q}_1} \cdot \frac{\partial}{\partial \vec{p}_1} + \frac{\vec{p}_1}{m} \cdot \frac{\partial}{\partial \vec{q}_1} \right] f_1 =  \int \! \diff V_2 \frac{\partial \mathcal{V}(\vec{q}_1 - \vec{q}_2)}{\partial \vec{q}_1} \cdot \frac{\partial f_2}{\partial \vec{p}_1},
\end{equation}
e
\begin{equation*}
\left[ \frac{\partial}{\partial t} - \frac{\partial \mathcal{U}}{\partial \vec{q}_1} \cdot \frac{\partial}{\partial \vec{p}_1} - \frac{\partial \mathcal{U}}{\partial \vec{q}_2} \cdot \frac{\partial}{\partial \vec{p}_2} + \frac{\vec{p}_1}{m} \cdot \frac{\partial}{\partial \vec{q}_1} + \frac{\vec{p}_2}{m} \cdot \frac{\partial}{\partial \vec{q}_2} - \frac{\partial \mathcal{V}(\vec{q}_2 - \vec{q}_1)}{\partial \vec{q}_1} \cdot \left( \frac{\partial}{\partial \vec{p}_1} - \frac{\partial}{\partial \vec{p}_2} \right)  \right] f_2  
\end{equation*}
\begin{equation}
= \int \! \diff V_3 \left[ \frac{\partial \mathcal{V}(\vec{q}_1 - \vec{q}_3)}{\partial \vec{q}_1} \cdot \frac{\partial}{\partial \vec{p}_1} + \frac{\partial \mathcal{V}(\vec{q}_2 - \vec{q}_3)}{\partial \vec{q}_2} \cdot \frac{\partial}{\partial \vec{p}_2} \right] f_3
\end{equation}
Si vuole ottenere un'equazione che consideri le interazioni a corto raggio tra le molecole.

[SPIEGARE COME CI SI ARRIVA]

Si consideri quindi l'equazione
\begin{equation}
\left[ \frac{\vec{p}_1}{m}\cdot\frac{\partial}{\partial \vec{q}_1} + \frac{\vec{p}_2}{m}\cdot\frac{\partial}{\partial\vec{q}_2} - \frac{\partial\mathcal{V}(\vec{q}_1-\vec{q}_2)}{\partial \vec{q}_1} \cdot \left( \frac{\partial}{\partial \vec{p}_1} - \frac{\partial}{\partial \vec{p}_2} \right)  \right] f_2 =0
\end{equation}

==> Chapters/Chapter5.tex <==
\section{ALTRO}

Essendo $\psi(\mathbf{x})\in L^2(\mathbb{R}^3)$, allora è possibile definire la trasformata di Fourier $\varphi(\mathbf{p})$ della funzione d'onda $\psi(\mathbf{x})$, definita da
\begin{equation}
\varphi(\mathbf{p}) = \bigintsss_{\mathbb{R}^3} \! \psi(\mathbf{x}) \frac{e^{-\frac{i}{\hbar} \mathbf{p}\cdot\mathbf{x}}}{(2\pi\hbar)^{3/2}} \, \diff \mathbf{x},
\end{equation}
ed è chiamata \textbf{funzione d'onda nello spazio degli impulsi}. Inoltre, per il Teorema di inversione di Fourier (cfr.~), è possibile scrivere $\psi(\mathbf{x})$ in termini di $\varphi(\mathbf{p})$ come l'anti-trasformata di Fourier di $\varphi(\mathbf{p})$, cioè
\begin{equation}
\psi(\mathbf{x}) = \bigintsss_{\mathbb{R}^3} \! \varphi(\mathbf{p}) \frac{e^{\frac{i}{\hbar} \mathbf{p}\cdot\mathbf{x}}}{(2\pi\hbar)^{3/2}} \, \diff \mathbf{p}.
\end{equation}
Si osservi che in questo modo $\psi(\mathbf{x})$ si può vedere come combinazione lineare di onde elementari del tipo 
\begin{equation}
\frac{e^{\frac{i}{\hbar} \mathbf{p}\cdot\mathbf{x}}}{(2\pi\hbar)^{3/2}}
\end{equation}
di impulso $\mathbf{p}$ fissato e aventi ampiezza $\varphi(\mathbf{p})$. Analogamente a quanto visto per la posizione, si può definire la densità di probabilità di impulso ponendo
\begin{equation}
\Pi(\mathbf{p})=\varphi^*(\mathbf{p})\varphi(\mathbf{p})=\vert \varphi(\mathbf{p}) \vert^2.
\end{equation}
Inoltre, per l'identità di Parseval, si ha che
\begin{equation}
\int_{\mathbb{R}^3} \! \vert \psi(\mathbf{x}) \vert^2 \, \diff \mathbf{x} =
\int_{\mathbb{R}^3} \! \vert \varphi(\mathbf{p}) \vert^2 \, \diff \mathbf{p},
\end{equation}
da cui si ottiene che
\begin{equation}
\int_{\mathbb{R}^3} \! \Pi(\mathbf{p}) \, \diff \mathbf{p}=1.
\end{equation}
Allora la funzione $\varphi(\mathbf{p})$ si chiama \textbf{funzione d'onda dello spazio degli impulsi}. Si osservi che lo spazio delle funzioni d'onda nello spazio degli impulsi è isomorfo allo spazio delle funzioni d'onda nello spazio delle coordinate. In esso può essere definito un prodotto scalare analogamente a quanto fatto prima con le funzioni d'onda nello spazio delle coordinate
\begin{equation}
\left\langle \varphi_1,\varphi_2 \right\rangle = \int_{\mathbb{R}^3} \! \varphi_1^*(\mathbf{p})\varphi_2(\mathbf{p}) \, \diff \mathbf{p}.
\end{equation}
\`{E} noto che la trasformata di Fourier conserva il prodotto scalare, cioè $\left\langle \psi_1,\psi_2 \right\rangle = \left\langle \varphi_1,\varphi_2 \right\rangle$. Quindi $\psi$ e $\varphi$ sono rappresentazioni equivalenti dello stesso stato.


\subsection{Richiami sulla teoria delle trasformate di Fourier}


\subsection{Deduzione del principio di indeterminazione}
Si consideri una particella in una dimensione e siano $\psi(x)$ e
\begin{equation}
\varphi(p) = \int_{-\infty}^{+\infty} \! \frac{e^{-\frac{i}{\hbar}px}}{\sqrt{2\pi\hbar}}\psi(x) \, \diff x
\end{equation}
le sue funzioni d'onda rispettivamente nello spazio delle coordinate e nello spazio degli impulsi. Interpretando $\vert \psi(x) \vert^2$ e $\vert \varphi(p) \vert^2$ come distribuzioni di probabilità, è possibile definire il \textbf{valore medio} della posizione e dell'impulso ponendo
\begin{equation}
\bar{x} = \int_{-\infty}^{+\infty} \! x \vert \psi(x) \vert^2 \, \diff x, \qquad
\bar{p} = \int_{-\infty}^{+\infty} \! p \vert \varphi(p) \vert^2 \, \diff p,
\end{equation}
e inoltre è possibile definire anche la loro varianza, qui indicate con $\Delta x$ e $\Delta p$ e dette \textbf{incertezza sulla posizione} e \textbf{incertezza sull'impulso}, ponendo
\begin{equation}
(\Delta x)^2 = \int_{-\infty}^{+\infty} \! (x-\bar{x})^2 \vert \psi(x) \vert^2 \, \diff x, \qquad
(\Delta p)^2 = \int_{-\infty}^{+\infty} \! (p-\bar{p})^2 \vert \varphi(p) \vert^2 \, \diff p.
\end{equation}
Allora si può dimostrare (cfr.~\citep{DISP:Papa}) che vale sempre
\begin{equation}
(\Delta x)^2(\Delta p)^2 \geq \frac{\hbar^2}{4}.
\end{equation}
\begin{teorema}[Relazione di indeterminazione di Heisenberg]
Sia $\psi\in L^2(\mathbb{R})$. Allora
\begin{equation}
(\Delta x)^2(\Delta p)^2 \geq \frac{\hbar^2}{4}.
\end{equation}
\end{teorema}
\begin{proof}
Per prima cosa si procede dimostrando il caso $\bar{x}=\bar{p}=0$. Allo scopo, si consideri
\begin{equation}
\int_{-\infty}^{+\infty} \! x \overline{\psi(x)}\psi ' (x) \,\diff x
\end{equation}
e si effettui una integrazione per parti, ottenendo
\begin{align*}
\int_{-\infty}^{+\infty} \! x \overline{\psi(x)}\psi ' (x) \,\diff x & = 
\left[ x \overline{\psi(x)} \psi(x) \right] _{-\infty}^{+\infty} -
\int_{-\infty}^{+\infty} \! \left( x\overline{\psi(x)} \right) ' \psi(x)  \,\diff x=\\
& = \left[ x \vert \psi(x) \vert^2 \right] _{-\infty}^{+\infty} -
\int_{-\infty}^{+\infty} \! \vert \psi(x) \vert^2 \,\diff x -
\int_{-\infty}^{+\infty} \! x \overline{\psi ' (x)}\psi(x) \,\diff x.
\end{align*}
\end{proof}
Essendo $x \vert \psi(x) \vert^2 \in L^2(\mathbb{R})$, allora $\left[ x \vert \psi(x) \vert^2 \right] _{-\infty}^{+\infty} =0$ e infine si ha che
\begin{align*}
1=\int_{-\infty}^{+\infty} \! \vert \psi(x) \vert^2 \,\diff x & = 
- \int_{-\infty}^{+\infty} \! x \overline{\psi(x)}\psi ' (x) \,\diff x 
- \int_{-\infty}^{+\infty} \! x \overline{\psi ' (x)}\psi(x) \,\diff x =\\
& = -2 \mathrm{Re} \int_{-\infty}^{+\infty} \! x\overline{\psi(x)}\psi'(x) \,\diff x.
\end{align*}
Elevando entrambi i membri al quadrato ed applicando la diseguaglianza di Cauchy-Schwarz si ottiene che
\begin{equation}
1\leq 4 \left( \int_{-\infty}^{+\infty} \! x^2\vert \psi(x) \vert^2 \,\diff x \right) \left( \int_{-\infty}^{+\infty} \! \vert \psi '(x) \vert^2 \,\diff x \right). 
\end{equation}
Infine, per il teorema di Plancherel, si ha
\begin{equation}
\int_{-\infty}^{+\infty} \! \vert \psi '(x) \vert^2 \,\diff x = 
\end{equation}






\subsection{Analisi spettrale}
Lo spettro è una delle caratteristiche più importanti di un operatore e rappresenta il collegamento tra la teoria degli operatori e moltissimi problemi della fisica.


\subsection{Autostati dell'hamiltoniana}
[AGGIUNGERE COSA MANCA]\\
Determinando un \textbf{insieme completo} di autofunzioni $\left\lbrace \phi_\lambda \right\rbrace_{\lambda\in\Lambda}$ nello spazio degli stati, è possibile rappresentare qualsiasi funzione d'onda $\psi$ come loro combinazione lineare, cioè
\begin{equation}\label{EQ:CAP1:Decomposizione_psi}
\psi = \sum_{\lambda\in\Lambda} a_\lambda \phi_\lambda.
\end{equation}
Si osservi che l'indice $\lambda$ identifica gli autostati ed è detto \textbf{indice quantico}, l'insieme $\Lambda$ è l'insieme in cui variano gli indici quantici. Se $\Lambda$ ha un numero finito di elementi, la definizione di insieme completo coincide con la definizione di base di uno spazio vettoriale.\\

[DEFINIRE AUTOVALORI ED AUTOSTATI]

L'insieme $\left\lbrace E_\lambda \mid \lambda\in\Lambda \right\rbrace$ degli autovalori dell'operatore $H$ si chiama \textbf{spettro} dell'operatore $H$. Se lo spettro non contiene alcun intervallo del tipo $\left] E_{\lambda_1},E_{\lambda_2} \right[$, lo spettro si dice \textbf{discreto} e spesso in tal caso gli autostati si indicano con un indice $n\in\mathbb{Z}$.

Nel caso in cui lo spettro non sia discreto, la somma \eqref{EQ:CAP1:Decomposizione_psi} su ogni intervallo contenuto nello spettro è da intendersi come integrale rispetto alla variabile continua $\lambda$.


\subsection{Osservabili}
\citep{DISP:Papa} pag. 71


Copia incolla da Anile-Mascali-Alì

Nella terminologia della meccanica quantistica, ogni quantità fisica per cui sia possibile effettuare una misurazione viene detta osservabile. Ogni osservabile è rappresentata da un operatore lineare autoaggiunto che agisce sullo spazio degli stati. Ogni autostato di un'osservabile corrisponde ad un preciso autovettore dell'operatore, e l'autovalore dell'operatore corrisponde al valore dell'osservabile di un sistema che si trova in quell'autostato. La probabilità che il risultato di una misurazione sia un certo autovalore è data dal modulo quadro del prodotto interno (il prodotto scalare dello spazio di Hilbert considerato) tra il vettore di stato prima della misurazione e il vettore corrispondente a quel dato autovalore del quale vogliamo conoscere la probabilità di presentarsi.

\subsection{Osservabili con spettri puntuali}
Si consideri un'osservabile $f$ con spettro puntale, i cui valori ammessi siano indicati con $f_n$, $n=0,1,2,\ldots$ e si consideri uno stato quantistico avente rappresentazione data dalle funzioni d'onda $\psi$, decomposte sugli autovettori $\psi_n$ dalla \eqref{EQ:CAP1:Comb_lin_funzioni_d_onda}. Si ha la seguente
\begin{definizione}
Si definisce \textbf{valore medio} (o \textbf{valore atteso}) di un'osservabile $f$ in un dato stato $\psi$, definito dalla \eqref{EQ:CAP1:Comb_lin_funzioni_d_onda}, la seguente quantità
\begin{equation}
\left\langle f \right\rangle = \sum_n f_n \vert a_n \vert ^2.
\end{equation}
\end{definizione}
Adesso bisogna introdurre l'operatore integrale $F$, formalmente definito su un vettore test $\phi\in L^2(\mathbb{R}^3)$ nel modo seguente
\begin{equation}
(F\phi)(\mathbf{x}) = \int_{\mathbb{R}^3} \! K(\mathbf{x},\mathbf{x}')\phi(\mathbf{x}') \, \diff \mathbf{x}',
\end{equation}
dove il nucleo $K$ è definito come
\begin{equation}
K(\mathbf{x},\mathbf{x}') = \sum_n f_n \psi^*_n(\mathbf{x}')\psi_n(\mathbf{x}).
\end{equation}
Allora, tale operatore agisce su $\psi$ nel modo seguente
\begin{align*}
(F\psi)(\mathbf{x}) & = \int_{\mathbb{R}^3} \! \sum_n f_n \psi^*_n(\mathbf{x}')\psi_n(\mathbf{x})\psi(\mathbf{x}') \, \diff \mathbf{x}'=\\
& = \sum_n f_n \psi_n(\mathbf{x}) \int_{\mathbb{R}^3} \! \psi^*_n(\mathbf{x}') \psi(\mathbf{x}') \, \diff \mathbf{x}' = \sum_n a_n f_n \psi_n \mathbf{x},
\end{align*}
dove l'ultimo passaggio si ottiene per la \eqref{EQ:CAP1:Def_coeff_stato_quantistico} e quindi si ha
\begin{equation}
\left\langle f \right\rangle = \left\langle \psi,F\psi \right\rangle. 
\end{equation}
\begin{osservazione}
L'operatore lineare $F$ è l'operatore formalmente associato all'osservabile $f$, il cui valore atteso $\left\langle f \right\rangle$ è definito dall'azione di $F$ sulla funzione d'onda dello stato quantistico.
\end{osservazione}
Allora ad ogni osservabile $f$ è possibile associare un operatore lineare auto-aggiunto $F$ sullo spazio di Hilbert  $L^2(\mathbb{R}^3)$. Questa procedure è detta \textbf{quantizzazione di un'osservabile}.

Si osservi che se la funzione $\psi$ è una delle autofunzioni $\psi_n$, allora $a_n=\delta _n ^{n'}$ e di conseguenza si ha
\begin{equation}
F\psi_n = f_n \psi_n,
\end{equation}
cioè i valori $f_n$ coincidono con gli autovalori dell'operatore lineare $F$ e le $\psi_n$ sono gli autovettori associati.
\begin{osservazione}
Poiché gli autovalori $f_n$ ed il valore medio $\left\langle f \right\rangle$ di una grandezza fisica sono numeri reali, allora l'operatore $F$ deve essere un operatore simmetrico, cioè
\begin{equation}
\left\langle \psi,F\phi \right\rangle = \left\langle F\psi,\phi \right\rangle, \quad \forall \psi,\phi\in L^2(\mathbb{R}^3).
\end{equation}
perché i suoi autovalori devono essere numeri reali. Tali operatori sono detti hermitiani o operatori simmetrici.
\end{osservazione}







\section{La struttura del grafene monostrato}

La grafite è una delle forme allotropiche del carbonio ed è la manifestazione macroscopica di uno dei più promettenti nano materiali di oggi. La struttura atomica della grafite è nota da tempo ed è oggetto di studi approfonditi. La grafite è un cristallo tridimensionale la cui struttura è a simmetria traslazionale esagonale, in cui si alternano due piani di esagoni. Non vi sono atomi al centro degli esagoni, per cui in ogni piano si hanno due sottoreticoli di traslazione. A metà distanza tra due piani che si sovrappongono vi è un altro piano di esagoni, ruotato di $\ang{60}$ rispetto ai piani adiacenti. In questo modo, in ogni centro dell'esagono del piano intermedio vi è un atomo nei piani adiacenti. La struttura appena descritta è rappresentata nella Figura [INSERIRE REF].



Studiando la grafite, si è osservato che i singoli strati sono delimitati solo debolmente dagli altri e ciò ha permesso la descrizione delle proprietà elettroniche della grafite come sistema bidimensionale già decenni fa senza tuttavia sembrare un sistema fisico di interesse.

La scoperta dei nanotubi di carbonio ha posto l'attenzione sui singoli strati che formano la grafite. Infatti, un nanotubo di carbonio è una fibra cava che costituisce un sistema monodimensionale e può essere visto come uno strato di grafite arrotolato, le cui proprietà elettroniche possono essere dedotte direttamente dai risultati bidimensionali per i singoli strati di grafite.

Il nome grafene per indicare un singolo strato di grafite è stato utilizzato per la prima volta nel 1987. Fin dagli anni '70 era noto come sviluppare i singoli strati di carbonio su vari substrati. Però il grafene indipendente ha proprietà elettroniche completamente diverse in quanto il singolo strato di carbonio interagisce fortemente con il substrato.

Fino alla prova sperimentale del contrario, si credeva, che proprio questa forte interazione con il substrato fosse necessaria per formare il grafene. Il gruppo di Andre Geim è stato Il primo a dimostrare che è possibile estrarre singoli fogli di grafene dalla grafite e metterli su un substrato, pur mantenendo le proprietà di un cristallo bidimensionale, formando il cosiddetto grafene libero.



Il grafene è un cristallo bidimensionale formato da un singolo strato di atomi di carbonio la cui struttura è un reticolo a celle esagonali.


Tale reticolo non è un reticolo di Bravais, perché...... Questa struttura può essere suddivisa in due sottoreticoli esagonali di Bravais con base biatomica.


%----------------------------------------------------------------------------------------




%----------------------------------------------------------------------------------------




%----------------------------------------------------------------------------------------




%----------------------------------------------------------------------------------------

\section{I modelli cinetici di trasporto}

[INSERIRE INTRO]




\subsection{La descrizione classica di un sistema di particelle elementari}

Si considerino un numero $N$ di elettroni in un solido e siano $\mathbf{x}_i$ e $\mathbf{k}_i$, $i=1,\ldots,N$, rispettivamente la posizione e il vettore d'onda della particella $i$-esima. Nell'approssimazione semiclassica, assumendo che le forze siano indipendenti da tutti i $\mathbf{k}_i$ e possano essere rappresentate da un campo gradiente con potenziale $\mathcal{U}(\mathbf{x}_1,\ldots,\mathbf{x}_N)$, il moto è ancora descritto da un sistema canonico con Hamiltoniana
\begin{equation}
\mathcal{H}(\mathbf{x}_1,\ldots,\mathbf{x}_N,\hbar\mathbf{k}_1,\ldots,\hbar\mathbf{k}_N)= \sum_{i=1}^N \mathcal{E}_i(\mathbf{k}_i) + \mathcal{U}(\mathbf{x}_1,\ldots,\mathbf{x}_N),
\end{equation}
ovvero
\begin{equation}\label{EQ:CAP1:Hamiltoniana_semiclassica}
\left\lbrace 
\begin{aligned}
\dot{\mathbf{x}}_i & = \frac{1}{\hbar} \nabla_{\mathbf{k}_i} \mathcal{H} \equiv \mathbf{v}_i\\
\dot{\mathbf{k}}_i & = -\frac{1}{\hbar} \nabla_{\mathbf{x}_i} \mathcal{H} \equiv \frac{1}{\hbar}\mathbf{F}_i
\end{aligned}
\right. \qquad i=1,\ldots,N
\end{equation}
con le condizioni iniziali
\begin{equation}
\mathbf{x}_i(0)=\mathbf{x}_i^0, \qquad \mathbf{k}_i(0)=\mathbf{k}_i^0.
\end{equation}



%----------------------------------------------------------------------------------------





\section{La materia allo stato solido}

[INSERIRE INTRO]

Si consideri un elettrone isolato. \`{E} possibile associare ad esso un vettore posizione $\mathbf{x}\in\mathbb{R}^3$ e un vettore velocità $\mathbf{v}\in\mathbb{R}^3$ con entrambi i vettori variabili al variare del tempo $t$.

[...]








%-----------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------

\section{TITOLO}

Si consideri un gas costituito da $N$ molecole monoatomiche. Si assume che lo stato di una molecola è determinato completamente dalle componenti del vettore posizione $\mathbf{x}$ e dalle componenti del vettore velocità di traslazione $\mathbf{v}$, si ignora cioè la possibile eccitazione dovuta ai gradi di libertà interni (rotazionale, vibrazionale ed elettronica). Si supponga che le molecole siano identiche. Se sono assegnate le posizioni e le velocità di tutte le molecole al tempo $t=0$, allora l'andamento successivo del sistema è determinato completamente dal sistema di $N$ leggi di Newton
\begin{equation}
m\frac{\diff^2 \mathbf{x}_k}{\diff t^2} = \mathbf{X}_k \qquad k=1,2,\ldots,N,
\end{equation}
dove $\mathbf{X}_k$ è la forza agente sulla $k$-esima molecola e $m$ è la massa di ciascuna molecola.

Nella pratica il numero di queste equazioni è enorme (in $1\,\si{\centi\metre}^3$ di gas a pressione atmosferica ci sono circa $10^{19}$ molecole). Quindi è opportuno procedere con una descrizione statistica dell'andamento del sistema.

Lo spazio a $6$ dimensioni in cui lo stato di una molecola è determinato dalle sue tre coordinate spaziali e dalle tre componenti della velocità è chiamato $\gamma$-spazio delle fasi o semplicemente $\gamma$-spazio. Il sistema delle $N$ molecole è rappresentato da $N$ punti di coordinate $(\mathbf{x}_i,\mathbf{v}_i)$ con $i=1,2,\ldots,N$.

Spesso è conveniente utilizzare uno spazio delle fasi a $6N$ dimensioni, detto $\Gamma$-spazio, in cui le coordinate sono le coordinate della posizione e le componenti della velocità di tutte le $N$ molecole. In questo spazio l'intero sistema delle $N$ molecole è rappresentato da un singolo punto.

Per definire lo stato desiderato di un sistema di molte particelle, si determina la probabilità di trovare il sistema in uno stato particolare. Sia
\begin{equation}
f_N(t,\mathbf{x}_1,\ldots,\mathbf{x}_N,\mathbf{v}_1,\mathbf{v}_N) \, \diff \mathbf{x}_1 \cdots \diff \mathbf{x}_N \, \diff \mathbf{v}_1 \cdots \diff \mathbf{v}_N
\end{equation}
la probabilità di trovare il sistema nei punti $(\mathbf{x}_i,\mathbf{v}_i)$ dello $\gamma$-spazio negli intervalli $\diff \mathbf{x}_i \, \diff \mathbf{v}_i$.

(..............)

La funzione di distribuzione $f(t,\mathbf{x},\mathbf{v})$ è di fondamentale importanza nella teoria cinetica dei gas. Tuttavia essa fornisce una descrizione inutilmente dettagliata perché dagli esperimenti è possibile calcolare solamente alcune quantità medie del gas, come la densità, la velocità, il tensore degli sforzi oppure il flusso di energia. Inoltre in molti problemi si è interessati solo a queste quantità medie.


\subsection{Gerarchia OLD}
Si supponga che le forze esterne possono essere espresse come la somma di un campo elettrico esterno e del potenziale di interazione a due particelle, cioè
\begin{equation}\label{EQ:CAP1:Potenziale}
\mathcal{U}(\mathbf{x}) = \sum_{i=1}^N \mathcal{U}\ap{ext}(\mathbf{x}_i) + \frac{1}{2} \sum_{\substack{i,j=1\\ i \neq j}}^N \mathcal{U}\ap{int}(\mathbf{x}_i,\mathbf{x}_j),
\end{equation}
con il potenziale di interazione simmetrico, cioè
\begin{equation}
\mathcal{U}\ap{int}(\mathbf{x}_i,\mathbf{x}_j)=\mathcal{U}\ap{int}(\mathbf{x}_j,\mathbf{x}_i).
\end{equation}
Questa scelta permette di dimostrare che la densità $P_N$ è indipendente dalla numerazione delle particelle, cioè esse risultano \textbf{indistinguibili} l'una dall'altra, ovvero
\begin{equation}\label{EQ:CAP1:Particelle_indistinguibili}
P_N(\mathbf{x}_1,\ldots,\mathbf{x}_N,\mathbf{k}_1,\ldots,\mathbf{k}_N,t)=P_N(\mathbf{x}_{\pi(1)},\ldots,\mathbf{x}_{\pi(N)},\mathbf{k}_{\pi(1)},\ldots,\mathbf{k}_{\pi(N)},t),
\end{equation}
per ogni permutazione $\pi$ di $\left\lbrace 1,\ldots,N \right\rbrace $, con $\mathbf{x}_i\in\mathbb{R}^3$, $\mathbf{k}_i\in\mathcal{B}$. Inoltre se la \eqref{EQ:CAP1:Particelle_indistinguibili} è verificata per $t=0$ allora essa è verificata per ogni $t$. \`{E} possibile introdurre la densità di probabilità congiunta per un sottoinsieme di $d$ particelle estratte da un insieme $N$ di particelle nel modo seguente
\begin{align*}
P_N^{(d)}(\mathbf{x}_1,\ldots,\mathbf{x}_d, & \mathbf{k}_1,\ldots,\mathbf{k}_d,t)=\\
&=\int_{(\mathbb{R}^3\times\mathcal{B})^{N-d}} \! P_N(\mathbf{x}_1,\ldots,\mathbf{x}_N,\mathbf{k}_1,\ldots,\mathbf{k}_N,t) \, \diff \mathbf{x}_{d+1} \diff \mathbf{k}_{d+1} \cdots \diff \mathbf{x}_{N} \diff \mathbf{k}_{N}.
\end{align*}
L'evoluzione delle $P_N^{(d)}$, con $1\leq d\leq N-1$, è governata dalla gerarchia BBGKY, che è una gerarchia di equazioni attribuita a Bogoliubov, Born, Green, Kirkwood e Yvon. Essa si ottiene integrando l'equazione di Liouville rispetto a $3(N-d)$ variabili di posizioni e vettori d'onda. Per fare ciò si consideri la seguente hamiltoniana
\begin{equation}
\mathcal{H}(\mathbf{x},\mathbf{p})=\sum_{i=1}^N\frac{\vert \mathbf{p}_i \vert^2}{2m} +\mathcal{U}(\mathbf{x})
\end{equation}
con $\mathcal{U}(\mathbf{x})$ dato dalla \eqref{EQ:CAP1:Potenziale}. Per valutare l'evoluzione nel tempo delle $P_N^{(d)}$, è opportuno suddividere l'hamiltoniana in
\begin{equation}
\mathcal{H}=\mathcal{H}_d+\mathcal{H}_{N-d}+\mathcal{H}',
\end{equation}
dove $\mathcal{H}_d$ e $\mathcal{H}_{N-d}$ includono le interazioni tra ogni gruppo di particelle, essendo
\begin{equation}\label{EQ:CAP1:H_d}
\mathcal{H}_d = \sum_{n=1}^d \left[ \frac{\vert \mathbf{p}_n \vert^2}{2m} + \mathcal{U}\ap{ext}\left( \mathbf{x}_n \right)  \right] + \frac{1}{2} \sum_{\substack{n,m=1\\ n \neq m}}^d \mathcal{U}\ap{int} \left( \mathbf{x}_n,\mathbf{x}_m \right),
\end{equation}
\begin{equation}\label{EQ:CAP1:H_N_d}
\mathcal{H}_{N-s} = \sum_{i=d+1}^N \left[ \frac{\vert \mathbf{p}_i \vert^2}{2m} + \mathcal{U}\ap{ext}\left( \mathbf{x}_i \right)  \right] + \frac{1}{2}  \sum_{\substack{i,j=d+1\\ i \neq j}}^N \mathcal{U}\ap{int} \left( \mathbf{x}_i,\mathbf{x}_j \right),
\end{equation}
e le interazioni tra le molecole contenute in
\begin{equation}\label{EQ:CAP1:H_primo}
\mathcal{H}'= \sum_{n=1}^d \sum_{i=d+1}^N \mathcal{U}\ap{int} \left( \mathbf{x}_n,\mathbf{x}_i \right).
\end{equation}
Dalla \eqref{EQ:CAP1:Densita_s_particelle} e dalla \eqref{EQ:CAP1:Liouville} si ha che l'evoluzione nel tempo delle $P_N^{(d)}$ può essere ottenuta calcolando
\begin{equation}\label{EQ:CAP1:Evoluzione_P_N_d}
\frac{\partial P_N^{(d)}}{\partial t} = \int \! \frac{\partial P_N}{\partial t} \, \prod_{i=d+1}^N \diff V_i = - \int \! \left\lbrace P_N,\mathcal{H}_d+\mathcal{H}_{N-d}+\mathcal{H}' \right\rbrace  \, \prod_{i=d+1}^N \diff V_i,
\end{equation}
in cui le parentesi di Poisson all'ultimo membro possono essere calcolate separatamente in virtù della proprietà \ref{PTA:CAP1:Parentesi_Poisson_pta_2} della Proposizione \ref{PROP:CAP1:Parentesi_Poisson}.





Poiché l'integrazione non riguarda le prime $d$ coordinate allora è possibile scambiare il segno di integrale e le parentesi di Poisson nel primo termine che si viene a creare applicando la proprietà \ref{PTA:CAP1:Parentesi_Poisson_pta_2} della Proposizione \ref{PROP:CAP1:Parentesi_Poisson} nella \eqref{EQ:CAP1:Evoluzione_P_N_d}, cioè si ha
\begin{equation}\label{EQ:CAP1:Evoluzione_H_d}
\int \! \left\lbrace P_N,\mathcal{H}_d \right\rbrace  \, \prod_{i=d+1}^N \diff V_i = \left\lbrace \left( \int \! P_N \, \prod_{i=d+1}^N \diff V_i \right),\mathcal{H}_d  \right\rbrace = \left\lbrace  P_N^{(d)},\mathcal{H}_d\right\rbrace .
\end{equation}
Per quanto riguarda il secondo termine della \eqref{EQ:CAP1:Evoluzione_P_N_d}, scrivendo esplicitamente le parentesi di Poisson e integrando successivamente per parti, si ottiene
\begin{equation}\label{EQ:CAP1:Evoluzione_H_N_d}
-\int \! \left\lbrace P_N,\mathcal{H}_{N-d} \right\rbrace  \, \prod_{i=d+1}^N \diff V_i = 0.
\end{equation}
Infine, per quanto riguarda il terzo termine della \eqref{EQ:CAP1:Evoluzione_P_N_d}, scrivendo esplicitamente le parentesi di Poisson, suddividendo la sommatoria, integrando per parti e semplificando si ha
\begin{equation}\label{EQ:CAP1:Evoluzione_H_primo}
-\int \! \left\lbrace P_N,\mathcal{H}' \right\rbrace \, \prod_{i=d+1}^N \diff V_i = (N-d) \sum_{n=1}^d \int \! \diff V_{d+1} \nabla_{\mathbf{x}_n} \mathcal{U}\ap{int}(\mathbf{x}_n,\mathbf{x}_{d+1}) \cdot \nabla_{\mathbf{p}_n} P_N^{(d+1)}
\end{equation}
(ulteriori dettagli su come ottenere \eqref{EQ:CAP1:Evoluzione_H_N_s} e \eqref{EQ:CAP1:Evoluzione_H_primo} sono presenti in \citep{BOOK:Kardar}).
Allora, sommando \eqref{EQ:CAP1:Evoluzione_H_s}, \eqref{EQ:CAP1:Evoluzione_H_N_s} e \eqref{EQ:CAP1:Evoluzione_H_primo} e sostituendo nella \eqref{EQ:CAP1:Evoluzione_P_N_d}, si ha
\begin{equation}\label{EQ:CAP1:Gerarchia_BBGKY_P_N}
\frac{\partial P_N^{(d)}}{\partial t} - \left\lbrace \mathcal{H}_d,P_N^{(d)} \right\rbrace = (N-d) \sum_{n=1}^d \int \! \diff V_{d+1} \nabla_{\mathbf{x}_n} \mathcal{U}\ap{int}(\mathbf{x}_n,\mathbf{x}_{d+1}) \cdot \nabla_{\mathbf{p}_n} P_N^{(d+1)}.
\end{equation}
Infine, scrivendo esplicitamente le parentesi di Poisson e ricordando che $\mathbf{p}_i=\hbar\mathbf{k}_i$ per ogni $i=1,\ldots,N$, si ottiene
\begin{equation}\label{EQ:CAP1:Poisson_H_d}
\left\lbrace \mathcal{H}_d,P_N^{(d)} \right\rbrace = \frac{1}{\hbar} \sum_{i=1}^d \left( \nabla_{\mathbf{x}_i} \mathcal{H}_d \cdot \nabla_{\mathbf{k}_i} P_N^{(d)} + \nabla_{\mathbf{k}_i} \mathcal{H}_d \cdot \nabla_{\mathbf{x}_i} P_N^{(d)} \right),
\end{equation}
in cui la sommatoria è estesa per $i=1,\ldots,d$ in quanto le funzioni che in essa compaiono sono nelle variabili $\mathbf{x}_1,\ldots,\mathbf{x}_d,\mathbf{k}_1,\ldots,\mathbf{k}_d$.
 
Per il calcolo del $\nabla_{\mathbf{x}_i} \mathcal{H}_d$ si osservi che nelle sommatorie della \eqref{EQ:CAP1:H_d} sopravvivono soltanto i termini che contengono $\mathbf{x}_i$ e inoltre si elimina il termine dipendente dai $\mathbf{p}_n$, ottenendo
\begin{equation}
\begin{aligned}
\nabla_{\mathbf{x}_i} \mathcal{H}_d & = \nabla_{\mathbf{x}_i} \mathcal{U}\ap{ext} (\mathbf{x}_i) +\frac{1}{2} \sum_{\substack{m=1\\ m \neq i}}^d  \nabla_{\mathbf{x}_i} \mathcal{U}\ap{int}(\mathbf{x}_i,\mathbf{x}_m) + \frac{1}{2} \sum_{\substack{n=1\\ n \neq i}}^d  \nabla_{\mathbf{x}_i} \mathcal{U}\ap{int}(\mathbf{x}_n,\mathbf{x}_i) =\\
 & = \nabla_{\mathbf{x}_i} \mathcal{U}\ap{ext} (\mathbf{x}_i) + \sum_{\substack{m=1\\ m \neq i}}^d  \nabla_{\mathbf{x}_i} \mathcal{U}\ap{int}(\mathbf{x}_i,\mathbf{x}_m)
\end{aligned}
\end{equation}
in cui l'ultima uguaglianza è ottenuta sfruttando la simmetria di $\mathcal{U}\ap{int}$. Inoltre in virtù delle [INSERIRE], si ha
\begin{equation}\label{EQ:CAP1:Grad_x_H_d}
\nabla_{\mathbf{x}_i} \mathcal{H}_d = -\mathbf{F}\ap{ext}(\mathbf{x}_i) - \sum_{\substack{m=1\\ m \neq i}}^d  \mathbf{F}\ap{int}(\mathbf{x}_i,\mathbf{x}_m).
\end{equation}
Per quanto riguarda il calcolo del $\nabla_{\mathbf{k}_i} \mathcal{H}_d$ si osservi che nella \eqref{EQ:CAP1:H_d} sopravvive solo il termine contenente $\mathbf{p}_i$, da cui, ricordando che $\mathbf{p}_i=\hbar\mathbf{k}_i$ e che $\mathbf{p}_i=m\mathbf{v}(\mathbf{k}_i)$, si ottiene
\begin{equation}\label{EQ:CAP1:Grad_k_H_d}
\nabla_{\mathbf{k}_i} \mathcal{H}_d = \nabla_{\mathbf{k}_i} \frac{\vert \hbar \mathbf{k}_i \vert^2}{2m} = \frac{\hbar^2}{m} \mathbf{k}_i = \hbar \frac{\mathbf{p}_i}{m} = \hbar \mathbf{v}(\mathbf{k}_i).
\end{equation}
Sostituendo le \eqref{EQ:CAP1:Grad_x_H_d} e \eqref{EQ:CAP1:Grad_k_H_d} nella \eqref{EQ:CAP1:Poisson_H_d} si ha
\begin{equation}\label{EQ:CAP1:Poisson_P_N_mod}
\begin{aligned}
\left\lbrace \mathcal{H}_d,P_N^{(d)} \right\rbrace = & - \frac{1}{\hbar} \sum_{i=1}^d \mathbf{F}\ap{ext}(\mathbf{x}_i) \cdot \nabla_{\mathbf{k}_i} P_N^{(d)} -\frac{1}{\hbar} \sum_{i=1}^d \sum_{\substack{j=1\\ j \neq i}}^d  \mathbf{F}\ap{int}(\mathbf{x}_i,\mathbf{x}_j)\cdot\nabla_{\mathbf{k}_i} P_N^{(d)}\\
&- \sum_{i=1}^d \mathbf{v}(\mathbf{k}_i) \cdot \nabla_{\mathbf{x}_i} P_N^{(d)}.
\end{aligned}
\end{equation}
Inoltre si consideri il secondo membro della \eqref{EQ:CAP1:Gerarchia_BBGKY_P_N}, osservando che
\begin{equation}
\nabla_{\mathbf{x}_n} \mathcal{U}\ap{int}(\mathbf{x}_n,\mathbf{x}_{d+1})=-\mathbf{F}\ap{int}(\mathbf{x}_n,\mathbf{x}_{d+1})
\end{equation}
e ricordando che $\mathbf{p}_n=\hbar\mathbf{k}_n$ si ottiene
\begin{equation}\label{EQ:CAP1:Gerarchia_BBGKY_mod}
\begin{aligned}
(N-d) \sum_{n=1}^d \int \! \diff V_{d+1} & \nabla_{\mathbf{x}_n} \mathcal{U}\ap{int}(\mathbf{x}_n,\mathbf{x}_{d+1}) \cdot \nabla_{\mathbf{p}_n} P_N^{(d+1)} =\\
&-\frac{1}{\hbar} (N-d) \sum_{n=1}^d \int \! \diff V_{d+1} \mathbf{F}\ap{int}(\mathbf{x}_n,\mathbf{x}_{d+1}) \cdot \nabla_{\mathbf{k}_n} P_N^{(d+1)}
\end{aligned}
\end{equation}
In definitiva, sostituendo la \eqref{EQ:CAP1:Poisson_P_N_mod} e la \eqref{EQ:CAP1:Gerarchia_BBGKY_mod} nella \eqref{EQ:CAP1:Gerarchia_BBGKY_P_N}, si ha
\begin{equation}\label{EQ:CAP1:Gerarchia_BBGKY}
\begin{aligned}
\frac{\partial P_N^{(d)}}{\partial t} & + \frac{1}{\hbar} \sum_{i=1}^d \mathbf{F}\ap{ext}(\mathbf{x}_i) \cdot \nabla_{\mathbf{k}_i} P_N^{(d)} + \frac{1}{\hbar} \sum_{i=1}^d \sum_{\substack{j=1\\ j \neq i}}^d  \mathbf{F}\ap{int}(\mathbf{x}_i,\mathbf{x}_j)\cdot\nabla_{\mathbf{k}_i} P_N^{(d)} \\
& + \sum_{i=1}^d \mathbf{v}(\mathbf{k}_i) \cdot \nabla_{\mathbf{x}_i} P_N^{(d)} \\
& + \frac{1}{\hbar} (N-d) \sum_{i=1}^d \int \! \diff V_{d+1} \mathbf{F}\ap{int}(\mathbf{x}_i,\mathbf{x}_{d+1}) \cdot \nabla_{\mathbf{k}_i} P_N^{(d+1)} =0.
\end{aligned}
\end{equation}
La \ref{EQ:CAP1:Gerarchia_BBGKY} è detta \textbf{gerarchia BBGKY}, attribuita agli scienziati Bogoliubov, Born, Green, Kirkwood e Yvon che per primi l'hanno studiata.


\subsection{Fondamenti matematici}

Si richiamano i concetti fondamentali della teoria della probabilità (...).

\begin{definizione}\label{DEF:Sigma_algebra}
Dato un insieme $\Omega$, una famiglia di insiemi $\mathcal{A}\subseteq\mathcal{P}(\Omega)$ si dice \emph{$\sigma$-algebra} se:
\begin{enumerate}
\item $\emptyset, \Omega \in \mathcal{A}$.
\item Se $A\in\mathcal{A}$ allora $A^C\in\mathcal{A}$.
\item Se $\lbrace A_i \rbrace_{i=1,2,\ldots} \subseteq \mathcal{A}$ allora $\bigcup_{i=1}^{\infty}A_i\in\mathcal{A}$.
\end{enumerate}
\end{definizione}

\begin{osservazione}\label{OSS:Sigma_algebra}
Dalla Definizione \ref{DEF:Sigma_algebra} e applicando la legge di De Morgan, si ha
\begin{equation*}
\bigcap_{i=1}^{\infty} A_i = \left( \bigcup_{i=1}^{\infty} A_i^C \right)^C 
\end{equation*}
e di conseguenza anche $\bigcap_{i=1}^{\infty} A_i \in \mathcal{A}$.
\end{osservazione}

\begin{definizione}
Sia $\Omega$ un insieme, $\mathcal{A}\subseteq\mathcal{P}(\Omega)$ una $\sigma$-algebra. Una \emph{probabilità} $P$ è un'applicazione $P:\mathcal{A}\rightarrow[0,1]$ tale che:
\begin{enumerate}
\item $P(A)\geq0 \quad \forall A \in \mathcal{A}$.
\item $P(\Omega)=1$.
\item Per ogni famiglia finita o numerabile $A_1,A_2,\ldots \in \mathcal{A}$ si ha
\begin{equation*}
P \left( \bigcup_{i=1}^{\infty} A_i \right) = \sum_{i=1}^\infty P(A_i) \qquad \mbox{se} \quad A_i \cap A_j = \emptyset \quad \forall i \neq j.
\end{equation*}
\end{enumerate}
\end{definizione}

\begin{definizione}
Si chiama \emph{spazio di probabilità} una terna $(\Omega,\mathcal{A},P)$ in cui: $\Omega$ è un insieme, $\mathcal{A}\subseteq\mathcal{P}(\Omega)$ è una $\sigma$-algebra e $P$ è una probabilità su $\mathcal{A}$.
\end{definizione}

\begin{definizione}
Dato uno spazio di probabilità $(\Omega,\mathcal{A},P)$ si dice \emph{variabile aleatoria} (v.a.) un'applicazione $X:\Omega\rightarrow\mathbb{R}$ tale che per ogni $a\in\mathbb{R}$ l'insieme $\lbrace \omega : X(\omega)\leq a \rbrace$ sia in $\mathcal{A}$.
\end{definizione}

\begin{osservazione}
Si può osservare che, se $X$ è una v.a. su uno spazio di probabilità $(\Omega,\mathcal{A},P)$, l'insieme $\lbrace \omega : X(\omega)> a \rbrace \in \mathcal{A}$ perché è il complementare dell'insieme $\lbrace \omega : X(\omega)\leq a \rbrace$ e dunque anche l'insieme
\begin{equation*}
\lbrace \omega : a<X(\omega)\leq b \rbrace = \lbrace \omega : X(\omega)\leq b \rbrace \cap \lbrace \omega : X(\omega)>a \rbrace
\end{equation*}
lo è, come intersezione di insiemi di $\mathcal{A}$. Allora, grazie all'Osservazione \ref{OSS:Sigma_algebra}, l'insieme $\lbrace \omega : X(\omega)=x \rbrace \in \mathcal{A}$ per ogni $x\in\mathbb{R}$, poiché è possibile ottenerlo come intersezione di insiemi di $\mathcal{A}$ mediante la relazione
\begin{equation*}
\lbrace \omega : X(\omega)=x \rbrace = \bigcap_{n=1}^{\infty} \lbrace \omega : x-\frac{1}{n}<X(\omega)\leq x \rbrace.
\end{equation*}
Per semplicità di notazione nel seguito si scriverà $\lbrace X\leq t\rbrace$, $\lbrace X\in A\rbrace$, $\ldots$ invece di $\lbrace \omega : X(\omega)\leq t\rbrace$, $\lbrace \omega :  X(\omega)\in A\rbrace$, $\ldots$
\end{osservazione}

\begin{definizione}
Data una v.a. $X$ si chiama \emph{funzione di ripartizione} (f.r.) la funzione $F_X : \mathbb{R}\rightarrow[0,1]$ definita da
\begin{equation*}
F_X(t)=P\lbrace X\leq t \rbrace.
\end{equation*}
\end{definizione}

\subsubsection*{Variabili aleatorie discrete}

\begin{definizione}
Una v.a. $X$ si dice \emph{discreta} se $X(\Omega)$ è un insieme al più numerabile e privo di punti di accumulazione.
\end{definizione}

\begin{definizione}
Data una v.a. discreta $X$ si chiama \emph{densità discreta} di $X$ una funzione $p:\mathbb{R}\rightarrow\mathbb{R}^+$ definita da
\begin{equation*}
p(x)=P\lbrace X=x \rbrace.
\end{equation*}
\end{definizione}

Si vuole estendere la definizione di v.a. al caso di applicazioni a valori in $\mathbb{R}^m$.

\begin{definizione}
Si definisce v.a. $m$-dimensionale discreta un'applicazione $X=(X_1,\ldots,X_m) : \Omega\rightarrow\mathbb{R}^m$ tale che le applicazioni $(X_1,\ldots,X_m)$ siano delle v.a. reali discrete.
\end{definizione}

\begin{osservazione}
Anche per una v.a. $m$-dimensionale discreta si può definire la \emph{densità discreta} ponendo
\begin{equation*}
p(x)=P\lbrace X=x \rbrace.
\end{equation*}
\end{osservazione}

\begin{definizione}
Se $X_1,\ldots,X_m$ sono v.a. reali discrete, la densità $p$ della v.a. $X=(X_1,\ldots,X_m)$ che è $m$-dimensionale, si chiama \emph{densità congiunta} delle v.a. $X_1,\ldots,X_m$.
\end{definizione}

\begin{definizione}
Se $X=(X_1,\ldots,X_m)$ è una v.a. $m$-dimensionale, le densità $p_1,\ldots,p_m$ delle v.a. $X_1,\ldots,X_m$ si chiamano \emph{densità marginali} di $X$.
\end{definizione}

\begin{definizione}
Date le v.a. discrete $X_1,\ldots,X_m$ definite su uno stesso spazio di probabilità, esse si dicono \emph{indipendenti} se e solo se per ogni scelta di $A_1,\ldots,A_m\subset\mathbb{R}$ si ha
\begin{equation*}
P\lbrace X_1\in A_1,\ldots,X_m\in A_m \rbrace = P \lbrace X_1 \in A_1 \rbrace \cdot \ldots \cdot P \lbrace X_m \in A_m \rbrace.
\end{equation*}
\end{definizione}

\begin{osservazione}
Sia $X$ una v.a. $m$-dimensionale e $\phi : \mathbb{R}^m \rightarrow \mathbb{R}^d$ una funzione. Allora $\phi(X)=\phi\circ X$ è ancora una v.a. ($d$-dimensionale).\\
Infatti, $\phi(X)$ assume i valori $\phi(x^{(1)})$,$\phi(x^{(2)})$,$\ldots$ che sono al più un'infinità numerabile (non tutti distinti se $\phi$ non è iniettiva). Inoltre, indicando con $y$ uno dei valori $\phi(x^{(1)})$,$\phi(x^{(2)})$,$\ldots$, allora
\begin{equation*}
\lbrace \phi(X)=y \rbrace = \lbrace X \in \phi^{-1}(y) \rbrace = \bigcup_{x \in \phi^{-1}(y)} \lbrace X=x \rbrace
\end{equation*}
e quindi $\lbrace \phi(X)=y \rbrace \in \mathcal{A}$ perché unione al più numerabile di elementi di $\mathcal{A}$ e ciò è equivalente ad affermare che $\phi(X)$ è una v.a.\\
Infine, si osservi che per definizione l'insieme $\phi^{-1}(y)$ è l'insieme di tutti i valori $x$ tali che $\phi(x)=y$ e quindi tale insieme è definito anche quando $\phi$ non è iniettiva e di conseguenza l'inversa $\phi^{-1}$ non esiste.
\end{osservazione}

\begin{definizione}
Sia $X$ una v.a. discreta che prenda i valori $x_1$, $x_2$,$\ldots$ e sia $p$ la sua densità. Si dice che $X$ ha \emph{speranza matematica finita} se
\begin{equation*}
\sum_i \vert x_i \vert p(x_i) <+\infty.
\end{equation*} 
In questo caso si chiama \emph{speranza matematica} di $X$ la quantità
\begin{equation*}
\mathbb{E}[X]=\sum_i x_i p(x_i) = \sum_i x_i P\lbrace X=x_i \rbrace.
\end{equation*}
\end{definizione}

\begin{definizione}
Sia $X$ una v.a. Per $k=1,2,\ldots$ si dice che $X$ ha \emph{momento di ordine $k$ finito} se la v.a. ha speranza matematica finita. In questo caso si chiama\emph{ momento di ordine $k$} della v.a. $X$ la quantità $\mathbb{E}[X^k]$. Analogamente se la v.a. $(X-\mathbb{E}[X])^k$ ha speranza matematica finita diremo che $X$ ha \emph{momento centrato di ordine $k$ finito} e si chiama \emph{momento centrato di ordine $k$} la quantità $\mathbb{E}[(X-\mathbb{E}[X])^k]$.
\end{definizione}

\begin{definizione}
Sia $X$ una v.a. che ha momento del secondo ordine finito. Si chiama \emph{varianza} il suo momento centrato del secondo ordine e si scrive
\begin{equation*}
VAR(X)=\mathbb{E}[(X-\mathbb{E}[X])^2].
\end{equation*}
\end{definizione}

\subsubsection*{Variabili aleatorie assolutamente continue}

\begin{definizione}
Una v.a. $X$ si dice \emph{continua} se la sua f.r. è una funzione continua.
\end{definizione}

\begin{definizione}
Una funzione $f:\mathbb{R}\rightarrow\mathbb{R}$ si dice \emph{densità} se e solo se $f\geq 0$, $f$ è integrabile su $\mathbb{R}$ e
\begin{equation*}
\int _{-\infty}^{+\infty} \! f(x) \,\diff x =1.
\end{equation*}
\end{definizione}

\begin{definizione}
Sia $X$ una v.a. continua, $F$ la sua f.r. e sia $f$ una densità. Si dice che $X$ \emph{ha densità} $f$ se
\begin{equation*}
F(x)=\int _{-\infty}^{x} \! f(t) \,\diff t
\end{equation*}
\end{definizione}

\begin{definizione}
Si dice che una v.a. $X$ è \emph{assolutamente continua} se $X$ è una v.a. che ha densità.
\end{definizione}


\section{ALTRO}
\subsection{INSERIRE NEL CAPITOLO 1 (Modello nucleare a shell)}\label{PAR:CAP1:Modello_shell}
Si definisce shell, una regione di spazio attorno al nucleo che può essere occupata da elettroni, corrispondente al numero quantico principale. Le shells definiscono la probabilità di trovare un elettrone in varie regioni di spazio relative al nucleo.

Le shells sono divise in subshells indicate con le lettere $s$, $p$, $d$ e $f$, ordinate per livelli di energia crescenti. Inoltre entro queste subshells, gli elettroni sono raggruppati in orbitali. Un orbitale è una regione dello spazio che contiene due elettroni ed ha uno specifico livello di energia quantizzato. La prima shell contiene un solo orbitale chiamato orbitale $1s$. La seconda shell contiene un orbitale $s$ e tre orbitali $p$ separati da angoli di $90^\circ$. Per questa ragione è possibile considerare gli orbitali $p$ orientati nelle direzioni degli assi $x$, $y$, e $z$. In definitiva, gli orbitali della seconda shell sono indicati con $2s$, $2p_x$, $2p_y$ e $2p_z$. Non saranno descritte le successive shells in quanto la configurazione elettronica degli elementi trattati in questa tesi si limita alla seconda shell.

La configurazione elettronica di un atomo è una descrizione degli orbitali occupati da ciascun elettrone. Ogni atomo ha un numero infinito di possibili configurazioni elettroniche. Per determinare quella a più bassa energia, detta \textbf{stato fondamentale}, si applicano le seguenti tre regole.
\begin{enumerate}
\item (Principio dell'Aufbau) Gli orbitali si riempiono in ordine crescente di energia.
\item (Principio di esclusione di Pauli) Soltanto due elettroni possono occupare un orbitale ed i loro spin devono essere opposti.
\item (Regole di Hund) La prima parte afferma che, se orbitali di eguale energia sono disponibili ma non ci sono abbastanza elettroni tali da riempirli tutti completamente, allora un solo elettrone viene aggiunto a ciascuno di tali orbitali, prima di aggiungere un secondo elettrone ad uno qualsiasi di essi. La seconda parte afferma che, gli spin dei singoli elettroni negli orbitali di eguale energia devono essere allineati.
\end{enumerate}
Ricordando che gli elettroni hanno carica negativa, il riempimento parziale degli orbitali avviene in modo tale da minimizzare il più possibile la repulsione elettrostatica tra gli elettroni. Se gli elettroni sono disposti con una configurazione diversa allora la sua energia sarà più alta e si avrà uno \textbf{stato eccitato}.

Gli elettroni posizionati nelle shells più esterne sono coinvolti nella formazione dei legami chimici. Tali elettroni sono detti \textbf{elettroni di valenza} e il livello energetico in cui essi si trovano è detto \textbf{livello di valenza}. Inoltre gli atomi interagiscono in modo da riempire il livello di valenza nei modi seguenti.
\begin{enumerate}
\item Un atomo può diventare uno \textbf{ione} se perde o guadagna elettroni in modo da completare il livello più esterno. L'atomo risulterà carico positivamente se perde elettroni, carico negativamente se li guadagna. Ioni di cariche opposte si attraggono e tale attrazione genera i cosiddetti \textbf{legami ionici}.
\item Un atomo può condividere elettroni con uno o più atomi per riempire il livello più esterno. Questo tipo di legame è detto \textbf{legame covalente}.
\item I legami possono essere in parte ionici e in parte covalenti. Questi legami sono detti \textbf{legami covalenti polari}.
\end{enumerate}

\subsection{INSERIRE NEL CAPITOLO 1 (Forma degli orbitali atomici $s$ e $p$)}\label{PAR:CAP1:Orbitali_s_p}
Tutti gli orbitali di tipo $s$ hanno la forma di una sfera, centrata nel nucleo atomico. Una rappresentazione tridimensionale degli orbitali $1s$ e $2s$ è mostrata nella Figura \ref{FIG:CAP2:orbitali_s}.
\begin{figure}[h]
\centering
\includegraphics[width=0.5\columnwidth]{Figures/Chapter2/orbitali_s.png}
\caption{Rappresentazione degli orbitali $1s$ (a sinistra) e $2s$ (a destra).}
\label{FIG:CAP2:orbitali_s}
\end{figure}
\FloatBarrier
Ogni orbitale $2p$ consiste di due lobi allineati con al centro il nucleo. Le direzioni dei tre orbitali di tipo $2p$ sono a due a due perpendicolari e sono indicati con $2p_x$, $2p_y$ e $2p_z$. Il segno della funzione d'onda è positivo in un lobo, zero nel nucleo e negativo nell'altro lobo. Questa rappresentazione è mostrata nella Figura \ref{FIG:CAP2:orbitali_p}.
\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{Figures/Chapter2/orbitali_p.png}
\caption{Rappresentazione degli orbitali $2p$.}
\label{FIG:CAP2:orbitali_p}
\end{figure}
\FloatBarrier
COMPLETARE pag. 29 \cite{BOOK:Organic-Chemistry}
\section{TITOLO}

La grafite è una delle forme allotropiche del carbonio ed è la manifestazione macroscopica di uno dei più promettenti nano materiali di oggi. La struttura atomica della grafite, con i suoi strati accatastati di reticoli esagonali di carbonio, è nota da tempo ed è oggetto di studi approfonditi. Si è presto osservato che i singoli strati esagonali sono delimitati solo debolmente dagli altri, consentendo così applicazioni di tutti i giorni, come la matita. Le proprietà elettroniche della grafite come sistema bidimensionale sono state studiate decenni fa ma non è mai stato considerato un sistema fisico di interesse.

La scoperta di fibre cave (nanotubi) di carbonio ha posto l'attenzione sui singoli strati che formano la grafite. Infatti, un nanotubo di carbonio può essere visto come uno strato di grafite arrotolato e le proprietà elettroniche di questo sistema monodimensionale possono essere dedotte direttamente dai risultati bidimensionali per i singoli strati di grafite.

I nanotubi di carbonio divennero presto un importante argomento di nanoscienza e tecnologia negli anni '90. Il nome grafene per indicare un singolo strato di grafite è stato utilizzato per la prima volta nel 1987. Monostrati di carbonio sviluppati su vari substrati erano conosciuti dagli anni '70, ma essi non sono considerati come il grafene indipendente, il quale ha proprietà elettroniche completamente diverse, rispetto a tali strati che interagiscono fortemente con il substrato.

Fino alla prova sperimentale del contrario, si credeva, che proprio questa forte interazione con il substrato fosse necessaria per formare il grafene. Il gruppo di Andre Geim è stato Il primo a dimostrare che è possibile estrarre singoli fogli di grafene dalla grafite e metterli su un substrato, pur mantenendo le proprietà di un cristallo bidimensionale, formando il cosiddetto grafene libero.
